Production of light stringy states

We discuss the direct production of light stringy states. Those states correspond to the lightest stringy excitations localized at the intersection of two D-brane stacks and their mass can be parametrically smaller than the string scale. Thus in a low string scale scenario one may observe stringy signatures at LHC even in the absence of the usual string resonances. We compute the tree level string scattering amplitude involving two gauge bosons and two such light stringy states. We give the squared amplitude summed over all polarization and gauge configuration and eventually apply the result to the quark sector of a D-brane realization of the Standard Model.

==> macro.tex <==
%\usepackage{a4}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{lscape}
\usepackage{cite}
\usepackage{epsfig}
\usepackage{multirow}
%\usepackage{psfig}
\usepackage[all]{xy}
\usepackage{amsmath}
%\usepackage{cite}
%\usepackage[dvips]{geometry}
%\usepackage{lscape}


\DeclareMathOperator{\ch}{ch} \DeclareMathOperator{\ck}{c}
\DeclareMathOperator{\dP}{dP} \DeclareMathOperator{\rank}{rank}

%\def\epsfig{\psfig}
\author{}


% draw box with width #1pt and line thickness #2pt
\newcommand{\drawsquare}[2]{\hbox{%
\rule{#2pt}{#1pt}\hskip-#2pt%  left vertical
\rule{#1pt}{#2pt}\hskip-#1pt%  lower horizontal
\rule[#1pt]{#1pt}{#2pt}}\rule[#1pt]{#2pt}{#2pt}\hskip-#2pt%  upper horizontal
\rule{#2pt}{#1pt}}% right vertical
% Young tableaux
\newcommand{\fund}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  fund
\newcommand{\Ysymm}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
         \raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  symmetric second rank
\newcommand{\Yasymm}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
        \raisebox{3pt}{\drawsquare{6.5}{0.4}}}%  antisymmetric second rank
\newcommand{\antifund}{\overline{\fund}}
\newcommand{\bYasymm}{\overline{\Yasymm}}
\newcommand{\bYsymm}{\overline{\Ysymm}}


\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\mbb}{\mathbb}
\newcommand{\ti}{\times}
\newcommand{\half}{\frac{1}{2}}
%\newcommand{\1}{{\bf 1}}
\newcommand{\3}{{\bf 3}}
%\newcommand{\2}{{\bf 2}}
%\newcommand{\24}{{\bf 24}}
%\newcommand{\10}{{\bf 10}}
\newcommand{\4}{{\bf 4}}
\newcommand{\5}{{\bf 5}}
\newcommand{\6}{{\bf 6}}
\newcommand{\8}{{\bf 8}}
\newcommand{\ergo}{$\Rightarrow$}
\newcommand{\ov}{\overline}
\def\IR{\relax{\rm I\kern-.18em R}}
\def\o#1{\overline{#1}}
\def\IP{\relax{\rm I\kern-.18em P}}
%\def\IC{\relax{\rm I\kern-.48em C}}
\def\inbar{\vrule height1.5ex width.4pt depth0pt}
\def\IC{\relax\,\hbox{$\inbar\kern-.3em{\rm C}$}}



\newcommand{\Z}{\mathbb{Z}}


\def\cn{{\cal N}}
\def\cm{{\cal M}}
\def\ca{{\cal A}}
\def\eps{\epsilon}
\def\T{{\bf T}}
\def\P{{\bf P}}
\def\K3{{\bf K3}}
\def\Om{\Omega}
\def\om{\omega}
\def\th{\theta}
\def\Th{\Theta}
\def\G{\Gamma}
%\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
%\def\i{\iota}
\def\sig{\sigma}
\def\car{{\cal R}}
\def\ov{\overline}
\def\preal{{\rm Re\,}}
\def\pim{{\rm Im\,}}
\def\raw{\rightarrow}
\def\longraw{\longrightarrow}
\def\n2d{\cN_{V^*}^{\otimes 2}}
\def\sCav{\overline{c}_{\av^*}}

\def\End{\mbox{End}}
\def\IC{\mathbb{C}}
%\def\II{\mathbb{I}}
\def\IE{\mathbb{E}}
\def\IQ{\mathbb{Q}}
\def\IR{\mathbb{R}}
\def\IF{\mathbb{F}}
\def\IZ{\mathbb{Z}}
\def\IO{\mathbb{O}}
\def\IP{\mathbb{P}}
\def\IH{\mathbb{H}}
\def\IK{\mathbb{K}}
\def\coker{{\mathop {\rm coker}}}
\def\Hom{{\rm Hom}}
\def\dim{{\rm dim}}
\def\cN{{\mathcal N}}
\def\cM{{\mathcal M}}
\def\cE{{\mathcal E}}
\def\cS{{\mathcal S}}
\def\cO{{\mathcal O}}
\def\cC{{\mathcal C}}
\def\cF{{\mathcal F}}
\def\cP{{\mathcal P}}
\def\cL{{\mathcal L}}
\def\nn{\nonumber}
\def\td{\mbox{td}}
\def\ch{\mbox{ch}}
\def\rk{\mbox{rk}}
\def\ind{\mbox{ind}}
\def\dirac{\slash{\! \! \! \! D}}
\newcommand{\gen}[2]{{\rm span}_{#1}\left\{#2\right\}}
\def\point{\mbox{pt}}
\def\av{\wedge^2 V}
\def\vv{V \otimes V^*}
\def\Tr{{\mathop {\rm Tr}}}
%\def\theequation{\thesection.\arabic{equation}}
\def\to{\rightarrow}
\def\sC{\bar{c}_U}
\def\im{\mathop {\rm im}}
\def\sym{{\rm Sym}}
\newcommand{\mat}[1]{\left( \matrix{#1} \right)}
\newcommand{\smat}[1]{{\scriptsize \mat{#1}}}
\newcommand{\tmat}[1]{{\tiny \mat{#1}}}
\def\II{{\rlap{1} \hskip 1.6pt \hbox{1}}}
%\newarrow{DotsTo}....>
%\newarrow{DDTo}{}{dash}{}{dash}>
\def\ol{\overline}
\def\navd{\cN_{\av^*}}

